A Large-Scale Study on the Usage of Testing Patterns that Address Maintainability Attributes (Patterns for Ease of Modification, Diagnoses, and Comprehension)

Test case maintainability is an important concern, especially in open source and distributed development environments where projects typically have high contributor turnover with varying backgrounds and experience, and where code ownership changes often. Similar to design patterns, patterns for unit testing promote maintainability quality attributes such as ease of diagnoses, modifiability, and comprehension. In this paper, we report the results of a large-scale study on the usage of four xUnit testing patterns which can be used to satisfy these maintainability attributes. This is a first-of-its-kind study which developed automated techniques to investigate these issues across 82,447 open source projects, and the findings provide more insight into testing practices in open source projects. Our results indicate that only 17% of projects had test cases, and from the 251 testing frameworks we studied, 93 of them were being used. We found 24% of projects with test files implemented patterns that could help with maintainability, while the remaining did not use these patterns. Multiple qualitative analyses indicate that usage of patterns was an ad-hoc decision by individual developers, rather than motivated by the characteristics of the project, and that developers sometimes used alternative techniques to address maintainability concerns.

==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section we discuss the results we collected for our three research questions. 





